Magnon-mediated superconductivity on ferromagnetic wallpaper fermions

We study two-dimensional superconductivity mediated by magnetic fluctuations at the interface between a ferromagnetic insulator and the nonsymmorphic topological crystalline insulator with a fourfold-degenerate Dirac point, wallpaper fermion. We demonstrate that BCS pairing with zero center-of-mass momentum induces chiral $p$-wave superconductivity, and the Amperean pairing with center-of-mass momentum $2k_{\rm F}$ can give rise to a parity-mixed superconducting state. We find that the Amperean pairing exhibits a mixture of $s$-wave and $p$-wave components due to the multiband nature of the wallpaper fermion and the easy-axis anisotropy of the ferromagnetic insulator. Additionally, we find that the stability of the superconducting state with BCS and the Amperean pairing is governed by the easy-axis anisotropy.

==> App_eff_int.tex <==
The effective interaction for the wallpaper fermions is obtained by the Schrieffer-Wolff transformation as follows.
The transformed Hamiltonian is given by
\begin{align}
 H' = H_0 + \frac{1}{2} [H_{\rm e-m}, S],
 \label{eq:SW1}
\end{align}
with the hermitian operator $S$ that is the solution of the following equation
\begin{align}
 H_{\rm e-m} + [H_0, S] = 0.
\end{align}
The explicit form is given by
\begin{align}
 S = 
 \sum
 \frac{M_{\boldsymbol{kq}}^{\alpha mn} }{\xi_{n\boldsymbol{k}} - \xi_{m\boldsymbol{k}+\boldsymbol{q}} + \omega_{\alpha\boldsymbol{q}} }
 \tilde a_{\alpha\boldsymbol{q}}
 \psi_{m\boldsymbol{k}+\boldsymbol{q}}^\dagger
 \psi_{n\boldsymbol{k}}
 - \mathrm{h.c.},
\end{align}
Equation (\ref{eq:SW1}) contains the four-fermion $H_{\rm eff}$, potential-scattering, and electron-magnon-scattering terms. 
\begin{align}
 H_{\rm eff}
 &= \frac{1}{2}
 \sum
 \frac{M_{\boldsymbol{kq}}^{\alpha nm} M_{\boldsymbol{k}'-\boldsymbol{q} \boldsymbol{q}}^{*\alpha m'n'} } {\xi_{m'\boldsymbol{k}'} - \xi_{n'\boldsymbol{k}'-\boldsymbol{q}} - \omega_{\alpha\boldsymbol{q}}}
 \notag\\&\hspace{5em}\times
 \psi_{n' \boldsymbol{k}'-\boldsymbol{q}}^\dagger
 \psi_{n \boldsymbol{k} + \boldsymbol{q}}^\dagger
 \psi_{m\boldsymbol{k}}
 \psi_{m'\boldsymbol{k}'}
 + \mathrm{h.c.},
 \notag\\&
 = \frac{1}{2} \sum
 V_{\boldsymbol{k} \boldsymbol{k}' \boldsymbol{q}}^{mm'nn'}
 \psi_{n' \boldsymbol{k}'-\boldsymbol{q}}^\dagger
 \psi_{n \boldsymbol{k} + \boldsymbol{q}}^\dagger
 \psi_{m\boldsymbol{k}}
 \psi_{m'\boldsymbol{k}'},
\end{align}
with
\begin{widetext}
\begin{align}
 V_{\boldsymbol{k} \boldsymbol{k}' \boldsymbol{q}}^{mm'nn'}
 &=
 \frac{1}{2}
 	M_{\boldsymbol{k},\boldsymbol{q}}^{\alpha nm} 
 	M_{\boldsymbol{k}'-\boldsymbol{q} ,\boldsymbol{q}}^{*\alpha m'n'}
 	\ab(
 	\frac{1}
 	 {\xi_{m'\boldsymbol{k}'} - \xi_{n'\boldsymbol{k}'-\boldsymbol{q}} - \omega_{\alpha\boldsymbol{q}}}
 	 -
 	 \frac{1}{
 	 	\xi_{m\boldsymbol{k}}
 	 -\xi_{n\boldsymbol{k}+\boldsymbol{q}} 
 	 + \omega_{\alpha \boldsymbol{q}}}
 	 )
 \notag\\&\quad
 + 
 \frac{1}{2}
 	M_{\boldsymbol{k}',-\boldsymbol{q}}^{\alpha n'm'} 
 	M_{\boldsymbol{k}+\boldsymbol{q}, -\boldsymbol{q}}^{*\alpha mn} 
 \ab(
 \frac{1}{
 \xi_{m\boldsymbol{k}} - \xi_{n\boldsymbol{k}+\boldsymbol{q}} 
 -\omega_{\alpha, -\boldsymbol{q}}
}
 -
 \frac{1}
 	{
 		\xi_{m'\boldsymbol{k}'} 
 		-\xi_{n'\boldsymbol{k}'-\boldsymbol{q}} 
 		+ \omega_{\alpha -\boldsymbol{q}}}
 	).
\end{align}
\end{widetext}
Note that the coupling constants satisfy the following relation, reflecting the Fermi-Dirac statistics.
\begin{align}
 V_{\boldsymbol{k}, \boldsymbol{k}', \boldsymbol{q}}^{mm'nn'}
 = 
 V_{\boldsymbol{k}', \boldsymbol{k}, -\boldsymbol{q}}^{m' m n'n}.
\end{align}





==> App_eff_int_iso_BCS.tex <==

Here, we consider the self-consistent equation for the BCS pairing 
\begin{align}
    \Delta_{\vv{k}} = -i\sum_{\vv{k}'} U_{\vv{k},\vv{k}'} \Delta_{\vv{k}},
\end{align}
where the $U_{\vv{k},\vv{k}'}$ is the real value coefficient corresponding to the imaginary part of the interaction matrix in our gap function.
Now we rewrite this equation, separating the real and imaginary parts as
\begin{align}
    \Re \Delta_{\vv{k}} 
    &= \sum_{\vv{k}'} U_{\vv{k},\vv{k}'} \Im \Delta_{\vv{k}},
    \notag \\
    \Im \Delta_{\vv{k}} 
    &= -\sum_{\vv{k}'} U_{\vv{k},\vv{k}'} \Re \Delta_{\vv{k}}.
\end{align}
Thus we find
\begin{align}
    \Re \Delta_{\vv{k}} 
     &= -\sum_{\vv{k}^\p,\vv{k}^{\p\p}} 
     U_{\vv{k},\vv{k}^\p}
     U_{\vv{k}^\p,\vv{k}^{\p\p}} \Re \Delta_{\vv{k}^{\p\p}}.
\end{align}
As the coefficient $U_{\vv{k},\vv{k}^\p}$, we suppose that $U_{\vv{k},\vv{k}^\p} = \sigma \vv{k}\cdot\vv{k}^\p$, 
where $\sigma \pm 1$.
According to this assumption, the self-consistent equation is given by
\begin{align}
    \Re \Delta_{\vv{k}} 
     &= -\sum_{\vv{k}^\prime,\vv{k}^{\prime\prime}} 
     (\vv{k} \cdot \vv{k}^\prime)
     (\vv{k}^\prime \cdot \vv{k}^{\prime\prime}) \Re \Delta_{\vv{k}^{\prime\prime}}.
\end{align}
Therefore, the self-consistent equation with pure imaginary value, which is odd for the inversion of $\vv{k}$, can not have non-trivial solutions.
Next, we consider the case that $U_{\vv{k},\vv{k}'} = \sigma \vv{k} \times \vv{k}'$.
In this case, we can see that
\begin{align}
    &\Re \Delta_{\vv{k}}
    \notag \\  
     &= -\sum_{\vv{k}^\prime,\vv{k}^{\prime\prime}} 
     (\vv{k} \times \vv{k}^\prime)
     (\vv{k}^\prime \times \vv{k}^{\prime\prime}) \Re \Delta_{\vv{k}^{\prime\prime}}.
\end{align}
Therefore, the terms of the cross-product, which are independent of the band index, enhance the odd parity solution, for example, chiral $p$-wave superconductivity.
The terms, which depend on the band index, also enhance the odd parity solution in specific combinations of the band index.
